Les Houches 2023: Physics at TeV Colliders: Standard Model Working Group Report

This report presents a short summary of the activities of the "Standard Model" working group for the "Physics at TeV Colliders" workshop (Les Houches, France, 12-30 June, 2023).

==> sm_pheno/sm_pheno.packages.tex <==
% add here the packages you used locally, 1 package per line

%\usepackage{xcolor}
%\usepackage{booktabs}
%\usepackage{arydshln}


==> tools/tools.packages.tex <==
% add here the packages you used locally, 1 package per line

%\usepackage{xcolor}
%\usepackage{booktabs}
%\usepackage{arydshln}

